Network Aware Compute and Memory Allocation in Optically Composable Data Centres with Deep Reinforcement Learning and Graph Neural Networks

Resource-disaggregated data centre architectures promise a means of pooling resources remotely within data centres, allowing for both more flexibility and resource efficiency underlying the increasingly important infrastructure-as-a-service business. This can be accomplished by means of using an optically circuit switched backbone in the data centre network (DCN); providing the required bandwidth and latency guarantees to ensure reliable performance when applications are run across non-local resource pools. However, resource allocation in this scenario requires both server-level \emph{and} network-level resource to be co-allocated to requests. The online nature and underlying combinatorial complexity of this problem, alongside the typical scale of DCN topologies, makes exact solutions impossible and heuristic based solutions sub-optimal or non-intuitive to design. We demonstrate that \emph{deep reinforcement learning}, where the policy is modelled by a \emph{graph neural network} can be used to learn effective \emph{network-aware} and \emph{topologically-scalable} allocation policies end-to-end. Compared to state-of-the-art heuristics for network-aware resource allocation, the method achieves up to $20\%$ higher acceptance ratio; can achieve the same acceptance ratio as the best performing heuristic with $3\times$ less networking resources available and can maintain all-around performance when directly applied (with no further training) to DCN topologies with $10^2\times$ more servers than the topologies seen during training.

==> problem_statement_long <==
\section{Problem Statemtent and Previous Work}

% NOTE: THIS SECTION CAN BE MASSIVELY IMPROVED/CUT:
% \begin{itemize}
%     \item less waffle conceptualising the problem and all it's possible scenarios - can potentially keep simplified version of the images but way shorter text
%     \item deeper explanation of why gnn/rl is compelling particularly for computer systems, include lots of references etc
%     \item point of the section is to conceptualise (just at a high level) why 1. EPS networks encounter fragmentation which could be avoided with resource disaggregation and 2. how careless allocation in resource disaggregated environments can return the fragmentation issue 3. motivate/indicate the combinatorial complexity of this problem and compel the reader that gnn/rl is a good way to do this.
% \end{itemize}

% EXTRA DETAIL REQUIRED:
% \begin{itemize}
%     \item request comes in asking for resources for an amount of time
%     \item disaggregated architecture means that resources are pooled in arbitrary quantities across numerous servers around the DC and then circuited together
%     \item these resources (node and network) are locked off to other requests until the one actively using them is finished
%     \item another advantage is device heterogeneity 
%     \item some things are simplified
%     \begin{itemize}
%         \item don't always know holding time of request
%         \item can have a variety of different resource distributions (e.g. heterogenous etc)
%         \item queuing is ignored for simplification
%         \item stochastic arrival is ignored (for same reason as queuing effectively)
%     \end{itemize}
% \end{itemize}



\subsection{Modern Data Centres and Fragmentation}

First will be shown an intuitive and simple example showing the resource fragmentation issue encountered in EPS-based DCs, motivating the need for disaggregated DCs and the problem addressed in this paper.

Fig. \ref{fig:eps_allocation} shows a simple DC-like network, which has 3 tiers of network switches (rack, aggregate and core) and a unique set of servers directly connected to each rack switch. Each server has 4 units of CPU resource, and 4 units of memory resource. The requests on the right are received in the order of top to bottom. The figure shows an instant in the lifetime of this system where the first request, needing to be split into smaller constituents that can each be placed onto a single server (as described in section \ref{section:intro}), has been divided into 4 sub-requests each placed on a unique server. Following this the second request must be placed. In terms of raw resource quantities, there is enough CPU and memory units available in the first rack (where the first request has been allocated) to satisfy this second request. However, some of the available memory units are in a server that has no available CPU units. As per the allocation restrictions due to EPS described earlier, these memory units are effectively stranded as they cannot be accessed by any CPU resources and are effectively useless. The second request, and any subsequent request at that, will never be able to use these memory resources until the first request finishes and releases it's resources. Furthermore, given its size, it will have to use resources from the second rack, potentially leading to further fragmentation in this part of the DC as well. This simple example serves to highlight the inherent inefficiency that is encountered when the backbone underlying a computer-network is unable to provide communication guarantees that can support remote resource access between distinct servers.


\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figs/eps_allocation.png}
    \caption{An EPS-based data centre. Since the red request is too large for a single server, it must be split into server-sized sub-requests, which can run in tandem and communicate over the network when necessary. Since resources must be pooled server-locally due to EPS-network communication limitations, however the purple request is allocated the leftover memory resources unused by the red request will be wasted (resource fragmentation).}
    \label{fig:eps_allocation}
\end{figure}

\subsection{Resource-Disaggregated Data Centres: Efficiency and Fragmentation}

% This paper explores the problem of developing an effective allocation agent that can handle network-aware resource allocation decisions in optically-disaggregated DCs. Described here at a high level, the problem consists of a optically-disaggregated DC, an allocator agent and a series of requests. Each requests specifies some amount of resources (this paper explores the case when servers consist of CPU and memory resources), and an amount of time that it needs them for. Furthermore, each request is only known when it arrives, not ahead of time. 

Here is considered the case when the underlying network can provide communication guarantees that are able to support inter-server resource pooling (i.e. it is resource disaggregated). While in principle the fragmentation problem discussed above can be avoided, there must be some additional consideration when making allocation decisions. When resources are allocated to an agent across multiple servers, there must be sufficient networking resources (i.e. optical circuits) available between these servers so that the network-enabled remote resource pooling described earlier can be implemented without detrimental effect on application performance. In the most extreme case (which is what is considered in this paper) there may need to be all-to-all connectivity between all servers involved in a single allocation. As such, sets of servers allocated to a particular request cannot be arbitrarily chosen. Rather, they must be chosen so ensure connectivity. Beyond this, they must be chosen to maximise the probability that connectivity can be found of other sets of servers that will be allocated and interconnected to other requests that arrive in the future, even when the exact form of those requests is not known in advance.

Re-addressing the allocation scenario addressed above, Fig. \ref{fig:nara_allocation_1} shows how the same two requests can be packed much more tightly into the first rack, leaving 100\% of the resources on the second rack free and effectively avoiding the fragmentation issue seen in the EPS-based DC. What is shown in Fig. \ref{fig:nara_allocation_1} is that, while the allocation of the first request still leaves some servers with memory units available but no server-local CPU resources to access them, these memory units can simply be pooled together with CPU units from other servers, provided that some network resources are available to do so (as shown by the red and purple lines representing links in the network). Avoiding resource fragmentation is not only useful for avoiding resource wastage, but also for reducing energy usage \cite{google dc power paper}. If a server is totally unused it can be operated in a low-energy standby mode, and kept this way until it needs to do active work. High resource fragmentation means that a higher than necessary number of servers need to be actively operated (not in low energy mode), even if they are only using a small portion of their total resources, incurring undue energy requirements.

However, there another form of fragmentation can be encountered in resource disaggregated DC systems if servers are chosen arbitrarily without careful consideration of the associated networking resources required (i.e. network awareness). Such a scenario is shown in Fig. \ref{fig:nara_allocation_2}. Here the system receives 3 requests, where the first two are the same as in the previous two examples. The first request is packed tightly into servers in the first rack only, as in Fig. \ref{fig:nara_allocation_1}, however the second request in this case is distributed across servers in both racks. There is nothing wrong with this choice in principle, however a consequence of this choice is that the second request requires a large amount of network resources to connect all of the servers involved in it's allocation across both racks. In the example shown here, this means that all of the networking resources used to communicate with the servers in the first rack are reserved for the second request since these servers must communicate with each other as well as the numerous servers in the second rack. Following this a third request is received. In terms of raw resource quantity, there are enough CPU and memory units in the first rack to satisfy this third request. Many of these units are located on the servers who are allocating some of their resources to the second request. However, since all of these servers' networking resources are reserved for the second request, there is no means for these resources to communicate beyond the server on which they are located. As such, these resources are once again effectively fragmented. Even though the network can in theory provide sufficient communication guarantees to allow for arbitrary resource pooling, a careless allocation strategy has rendered some resources unable to interact with this network.


\subsection{Challenges and Considerations of Network Aware Resource Allocation}



\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figs/nara_allocation_1.png}
    \caption{In a resource-disaggregated data centre requests can be more tightly packed into servers. Following Fig. \ref{fig:eps_allocation}, now the purple request can use the memory resources that are unused by the red request, but would otherwise be stranded on their local server since the CPU resources are occupied. This demonstrates how resource-disaggregation over the network can allow for more efficient allocation decisions.}
    \label{fig:nara_allocation_1}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figs/nara_allocation_2.png}
    \caption{Follows from Fig. \ref{fig:nara_allocation_2}. If placement decisions in resource-disaggregated data centres (which use both server and netwrok resources) are made haphazzardly, they will cause congestion in the network. This will then lead to another form of resource fragmentation whereby resources are unable to use networking resources to pool together with other non-local resources. The purple request has used all of the network between rack 1 and rack 2. This means that the blue request cannot be packed as efficiently across the two racks as if the networking resources were more carefully used.}
    \label{fig:nara_allocation_2}
\end{figure}

Co-allocation of server and network resources maps to an online case of the Quadratic Assignment problem, a canonical NP-hard combinatorial optimisation problem \cite{Meng2010}. This means that, especially for networks at the scale of modern DCNs, exact solutions are computationally intractable due to the complexity of the problem at this scale. Moreover, in the problem addressed in this paper, the problem is converted to an online version whereby resource requests arrive one at a time and must be allocated in that instant before another request is received. Furthermore the allocator only knows the form of the most recently arrived request, and does not know what request will arrive next or at any time in the future. In this sense the complexity of the problem is further increased. There is no strong notion of a globally optimal allocation here, since it isn't known ahead of time what needs to be allocated; will an `optimal' allocation now still be optimal when more requests have been received in the future? 

In general, these issues are standard when facing online problems with high combinatorial complexity (e.g. scheduling problems, routing problems etc). Heuristic solutions are often embraced where the trade-off between simplicity and solution quality is acceptable with respect to required system performance outcomes. For example, modern DC systems (which are not resource-dissaggregated) use often simple packing heuristics such as best-fit, worst-fit or dominant resource fairness as the algorithmic basis for their resource management platforms \cite{Ghodsi2011, Isard2009, Schwarzkopf2013, Verma2015, FacebookTupperware}. While these methods are certainly non-optimal, they provide the advantage of being both simple to implement and to understand, meaning that while they are not necessarily able to perform optimally, their shortcomings can be for the most part anticipated. Another avenue of heuristic design is to more actively craft a novel heuristic which is thought to be well customised for the task at hand. For example, one of the baselines used in this paper \cite{Yuan18} was designed specifically for the type of allocation problem addressed here and uses a combination of k-shortest paths (with weighting), breadth-first-search and a contention criteria to form a novel heuristic. While these more specialised methods can indeed provide better performance than more generic methods \cite{Zervas17,Yuan18}, they are non-intuitive to design due to the inherent complexity in the problem and are therefore typically subject to bias from the designer. Similarly, it is difficult to predict how these more complex hand-designed methods will perform in unseen environments and is also difficult in general to predict ahead of time how well a particular method will perform given some changes in the environment \cite{shabka21}.

Given the often unpredictable nature of data centre traffic as well and it's more gradually changing nature, a resource allocation technique for a resource disaggregated data centre architecture in the future should be all of the following. \textit{Scalable} with respect to network size; \textit{flexible} with respect to network structure/resource availability; \textit{efficient} with respect to long-term resource utilisation and acceptance rate. Furthermore, with respect to it's design, it is ideal if the method is built on minimal or no assumptions about the underlying network so it can avoid the design biases often encountered from other hand-desinged methods, and be more flexible under changing network environments.

\subsection{Solving Graph-Based Combinatorial Optimisation Problems with Deep Learning}

As noted, the problem addressed here is a NP-hard combinatorial optimisation. More specifically, the problem is one of this type which is defined on a graph (i.e. the DC topology). DRL with GNN-based policy functions, have been shown to be very effective in solving online variants of such problems. 

This method was first introduced in \cite{Dai2018} with respect to optimisation problems where solutions can be generated by iteratively selecting nodes in a topology until the set of chosen nodes satisfies (or violates) some kind of solution criteria. The high level node-selection pipeline of this method goes like: 
\begin{enumerate}
    \item A GNN processes the topology on which the problem is defined, outputting a distinct embedding for every node in the topology following it's message-passing and aggregation procedure.
    \item A RL agent takes an action, where an action is typically the act of adding a particular node in the topology to the solution set. The embedding representation of each node will be processed in some way by the RL agent in order to evaluate it's value/the likelihood of selecting that action, meaning that the agent is selecting nodes which themselves contain some information about their neighbouring nodes/edges.
    \item The selected node is added to the solution set. If a solution criteria is neither met nor violated by this set, the agent will choose another node until this is no longer the case.
\end{enumerate}

If training, then in accordance with standard DRL procedure the agent will receive a reward either when a full solution set has been generated (whether it was sucessful or not) or after each action (often termed intermediate rewards in this context). While a fundamental overview of this methodology is not provided here (it is clearly outlined in \cite{Dai2018}), section \ref{section:problem_spec} outlines how it has been adapted to the specific problem addressed in this paper.

Various following works show iterations or modifications of this general methodology, where different reinforcement learning algorithms, graph neural network architectures, or problem formulation principles are explored as a means of improving the performance, scalability and training or inference speed of such methods \cite{Zhuwen2018, Akash2019, barrett19}. Similarly, while initially topologically inflexible and relatively slow to train, many numerous advancements in GNN architecture design have vastly improved the ability for GNNs to be applied to very large graphs, be topologically flexible (i.e. applicable on inference to different topologies to those seen during training), and accurate \cite{Velickovic2018, Hamilton2017, Kipf2017}. Furthermore, alongside this fundamental methodological development, there have been various demonstrations of this methodology providing compelling advantages for similar problems in various domains including cluster scheduling and optical network routing \cite{shabka21, Mao2016, Mao2019, Almasan2019}. Generally, while the specific problem criteria and experiments differ across these various applied works, the advantages of applying this methodology can typically be summarised as:

\begin{enumerate}
    \item The learnt method is more flexible under variations in the optimisation environment, and should the environment change significantly it can simply be retrained rather than fully re-designed.
    \item The GNN-architecture choice can offer considerable scalability with respect to the size of graphs that can be handled and how fast a solution set can be constructed.
    \item The GNN-architecture choice can also offer considerable flexibilty with respect to the shape of the topology that is seen on inference vs during training.
    \item Treating the problem as a DRL problem means that the policies learnt can be long-sighted rather than greedy.
    \item Well designed, generic and high-level goal focused reward functions can be leveraged to yield fair policies (e.g. prioritising certain types of requests to the neglect of other types). 
\end{enumerate}

As such, this methodology lends itself very nicely to the problem addressd here, which can be solved by choosing servers to allocate to a request until either the request has enough resources, or the inter-server connectivity requirement fails. The following section describes how this problem is formulated as a markov decision process so that it can be solved by the aforementioned GNN-based DRL methodology for online graph-based combinatorial optimisation problems.
